On Democracy in Peer-to-Peer systems

The information flow inside a P2P network is highly dependent on the network structure. In order to ease the diffusion of relevant data toward interested peers, many P2P protocols gather similar nodes by putting them in direct contact. With this approach the similarity between nodes is computed in a point-to-point fashion: each peer individually identifies the nodes that share similar interests with it. This leads to the creation of a sort of "private" communities, limited to each peer neighbors list. This "private" knowledge do not allow to identify the features needed to discover and characterize the correlations that collect similar peers in broader groups. In order to let these correlations to emerge, the collective knowledge of peers must be exploited. One common problem to overcome in order to avoid the "private" vision of the network, is related to how distributively determine the representation of a community and how nodes may decide to belong to it. We propose to use a gossip-like approach in order to let peers elect and identify leaders of interest communities. Once leaders are elected, their profiles are used as community representatives. Peers decide to adhere to a community or another by choosing the most similar representative they know about.

==> Conclusions.tex <==
In this paper we proposed AP$2$PLE, an asynchronous peer-to-peer leader election algorithm. Its aim is to identify, in a peer to peer fashion, a set of leaders representing user communities. A leader is a peer elected by a set of other peers as their representative on the basis of their similarity with it.
The approach is based on peer-to-peer epidemic protocols for spreading information about network nodes. 
Each peer is associated with a network user, and is characterized by a profile. The leader's profiles is used as the community identifier. 
The election mechanism allows both the gathering into communities and the determination of the community leaders. 
Starting from the ``private'' vision of each node, after successive interactions and exchange of information among peers, it allows to exploit each peer local knowledge to contribute to the identification of the community leaders.  


==> Introduction.tex <==
What do people want to know? This is a very hard question to answer, probably it is impossible to give an universal answer 
due to different interests different groups of people are interested to. It is possible that who is reading this paper wants to know about the last Steve Jobs keynote, whereas other persons want to gather all the available information about the last car released by BMW. These different willings lead people to build specific connections (or better, strike up friendships) with other people on the basis of common shared interests. These ``connections'' make possible the human social behavior of spreading knowledge by exchanging  information between people that are in direct contact, in other words the human activity also known as \textit{word-of-mouth}. This well known phenomena has inspired the \textit{automating the word-of-mouth}~\cite{WOM} approach. A very effective solution that aims to exploit collaborative and social information for filtering data. In particular, in its first formulation has been exploited to filter information such as music albums and artists. 
%
However, after the publication of \cite{WOM}, several other systems (mainly centralized) like search engines (e.g. Yahoo!, Google or Bing), as well as some online stores (e.g. Amazon, eBay) have been exploited the concept behind the~\cite{WOM} paper. Indeed, in a world where there is a growing need to rapidly access and be aware of many types of distributed resources like Internet pages, shared files, online products, news and information, a flexible and efficient mechanism as \cite{WOM} is, exhibits relevant social and economic impacts. However, despite its effectiveness, scalability concerns are always related with these type of approaches.
%
Along the years, in order to address these scalability issues, several approaches has been proposed. Beyond the obvious parallelization of the approach, that in this case remains centralized. One of the most promising alternatives is the P2P approach. Peer-to-peer solutions scale well to large numbers of peers and deal gracefully with system dynamism, whereas centralized systems need expensive and complex techniques to ensure continuous operation under node and link failures. P2P systems are implemented through the collaboration of the peers without needing any centralized authority that would store all the user data.

Among the different approaches based on the peer-to-peer paradigm, the ones exploiting the Gossip~(\cite{PeerSampling1,PeerSampling2}) technique looks very promising. These protocols stems from their ability to reliably pass information among a large set of interconnected nodes, even if the nodes join and leave the system. Furthermore, as the name suggests, these protocols model in a very close way the behavior of people. Indeed, according to the gossip-based protocol, each node in the network periodically exchanges information with a subset of other peers. The choice of this subset (the peer community) is crucial to the proper dissemination of the gossip. An example exploiting such paradigm is the one we presented in~\cite{paperoCIT2010}. It proposed an architecture for a system that exploits the collaborative exchange of information between peers in order to allow them to build a proper neighborhood sharing common interests. 
The ultimate aim of the paper was to allow to each peer to build a neighborhood 
with which to exchange information, suggestions and recommendations based on the \textit{word-of-mouth} concept. 
%
With this approach the similarity between nodes is computed in a point-to-point fashion: each peer individually identifies the nodes that share similar interests with it and stores in its neighborhood the set of closer peers it found in the network so far. This leads to the creation of a sort of ``private'' communities, limited to each peer neighbors list. This ``private'' knowledge do not allow to identify the features needed to discover and characterize the correlations that collect similar peers in broader groups. 
%
In order to let these correlations to emerge, the collective knowledge of peers must be exploited.  In order to avoid the ``private'' vision of the network, the main problem to overcome is related to how to determine, in a distributed fashion, the representation of a community as well as to decide how nodes may choose to join that community. 
%
To address this limitation, in this paper we propose AP$2$PLE (Asynchronous Peer-to-Peer Leader Election), an approach that allows peers to create explicit  communities. The approach is based on the identification and the election of communities leaders.
Once a leader has been elected, its profile is used as community representation. It is worth to point out that the role of the leader is just to give to the leaded community a recognizable representation (i.e. the leader is NOT a SuperPeer). By using this representation the non-leader peers can decide to adhere to a community or another by comparing their profile against the leader ones. At the end, they will belong to the community represented by the leader with which they share the highest profile similarity.

The remaining of this paper is organized as follows:

Section~\ref{sec:RelatedWork} describes the solutions already present in the literature.
Section~\ref{sec:ProblemDescription} describes the problem we address in this paper.
Section~\ref{sec:TheProposedSolution} presents a detailed description of our solution.
Section~\ref{sec:TheProtocolInAction} presents a step-by-step example describing the algorithm behavior. 
 Finally, Section~\ref{sec:Conclusions} presents conclusions and considerations about this work.




==> ProblemDescription.tex <==
Networks of entities (e.g. humans, peers, ...) have enlightened to have emerging structures, embodied in the relationships among their participants. The properties of these structures, or communities,  are of the most importance to guarantee a fast and efficient communication among entities.

In order to discover those relationships, the main problems are the identification and representation of these structures. Consider a scenario of a set of entities. Every entity has a group of different profiles, each representing a different interest. Generally, one common solution, for every distinct interest,  is to partition to whole set of entities into groups showing a good grade of homogeneity. 

More  formally, given a set $\mathscr{N}_I$ of entities, for the interest $I$, we want to have a partition:

$$\mathscr{N}_I = \{N_1, \ldots, N_s\}$$

\noindent where each $N_i$ contains a homogeneous subset of the entities in $\mathscr{N}_I$. 

This goal implies to have a tradeoff on the cardinality of such groups. Larger groups could have too little internal correlation between members, whereas smaller groups could be too elitist, failing to catch existing relationships with members of other groups.

Moreover, for each $N_i \in \mathscr{N}_I$, we wish to find a proper label $e_i$ that gives an easy and immediate way to detect the membership to the group and to recognize its content. 

All the above issues are make even harder in distributed, dynamic environments like Peer-to-Peer (P2P) networks. This kind of networks is characterized by  the lack of global knowledge, a high number of participating peers and a high grade of changes due to join/leave operations performed unpredictably by each node. 

In order to face those problems, many approaches try to gather similar nodes by putting them in direct contact. This behavior allows each node to store the most similar other peers it encounters during message exchanges with other nodes. On of the most significant limitations of this approach is that similarity of interests between nodes is computed in a point-point fashion. In other words, each peer individually computes which are the other nodes that may share similar content/interest with it. This leads to the creation of a sort of  ``private'' communities, limited to each peer neighbor list.  This ``private'' knowledge  do not allow to give a good identification of   the features needed to characterize such communities, since it does not give any recognizable identifier for communities of similar peers, thus failing to reach the goal stated at the beginning of this section.

Thus, a more extended collaboration between peers has to be exploited in order to form a collective agreement over communities and community representatives.


==> RelatedWork.tex <==

In the past several solutions have been proposed for distributing data over an overlay P2P network to enable better resource tracings and better connectivity between similar elements. Such solutions exploit different techniques such as Gossip \cite{gosskip, proactive_mgmt_p2p, paperoCIT2010, PeerSampling1, PeerSampling2, Gossple}, Semantic Overlay Network \cite{son}, Election-based mechanism \cite{leader_election_adhoc, RanLeEl}.

In \cite{gosskip} the GosSkip systems is proposed. It is a self organizing and fully distributed overlay that provides a support to data storage and retrieval in peer-to-peer environments. It links objects rather than computational entities in a structure formed by a set of balanced trees. GosSkip is built using a gossip-based protocol that organizes peers so that they form an ordered double-linked list (or ring).
In GosSkip a peer is associated with a single item of data, and it is managed by the physical node that published the item. Each peer has a name that describes the semantics of the object to which is associated. The only property needed is that these names follow a total and deterministic order. So, the position of an element is fully determined by its name. For the information distribution, it exploits an epidemic-based protocol that maintains $O(log(N))$ peer states, and with a routing cost of $O(log(N))$.

To associate links to published object can lead to a very large number of connections. This is especially true in networks where the number of objects shared by each user is large. For example, networks for media sharing. Furthermore, using GosSkip it is difficult to search not knowing the exact name which identifies the item you are looking for.

The aim of the study conducted in \cite{son} is to reduce the search time of queries executed in peer-to-peer networks that create the overlay
network randomly, and at the same time to maintain a high degree of autonomy of the nodes. The authors propose node connections influenced by content, so that, for example, nodes having many ``Jazz'' files will connect to other similar nodes. Thus, semantically related nodes form a Semantic Overlay Network (SON). The overlay network is organized in SONS, i.e. a tree where each node consists of clusters of peers. 
Queries are routed to the appropriate SONs, increasing the chances that matching files will be found quickly, and reducing the search load on nodes that have unrelated content.
The SON-based overlay networks have a rigid predefined structure. The overlay network does not allow a dynamic reorganization of itself and leads to have 
clusters of not semantically related node also when solutions structured in multiple levels that can mitigate this disadvantage are exploited.

The paper \cite{semanticpeer} proposes the Peer Data Management System (PDMS) as a solution to the problem of large-scale sharing of semantically rich data. A PDMS consists of semantic peers connected through semantic mappings. Querying a PDMS may lead to poor results because of semantic degradation caused by the approximations provided during the construction of semantic mappings, which raises the problem of how to promote a mapping of the network in PDMS. The authors propose a strategy for incrementally maintenance a flexible network organization that clusters together peers, which are semantically related in SONs also guaranteeing a high degree of node autonomy. The lack of a common dictionary between peers may lead to similar content even if not the same, but described with the same concepts. To resolve this heterogeneity nodes with semantically similar concepts are grouped in the same SON. 
A critical aspect of this solution is the evolution of the interests of a peer that leads in changing the concepts it represents. This aspect introduces overheads in the maintenance of the SONs because changes involve changes in the structure of the network that are made through complex procedures. In fact, changes in a peer concepts triggers a distributed mechanism to reorganize the overlay network that involves to all the neighbor peers belonging to the related SONs. 

In \cite{proactive_mgmt_p2p} a proactive method to build a semantic overlay is proposed. Such approach is structured according to two layers. The top layer exploits the Vicinity \cite{vicinity} gossip-based protocol to optimize semantic lists for searching only. The bottom layer offers a fully decentralized service for delivering information on new events. At this level the Cyclon \cite{Cyclon} protocol is used to uniformly and randomly select peer throughout the network. Such peers are then passed to Vicinity to make lists of semantic peers. To form such lists the peer clustering is done in a completely implicit way, i.e. without requiring the user to specify any preferences or to characterize the content of files being shared. The conducted evaluation carried out that such lists are highly effective when searching for content. The construction of these lists through epidemics is efficient and robust, even in the presence of changes in the network.
A disadvantage of this solution consists in the fact that the clustering of the concepts could lead to reduce the reachability between peers. Each peer is semantically related only to the similar ones, this can lead to divide peer into compartments isolated from each other. The lack of an overall or distributed structure describing the state of the network does not allow a global routing query.

The paper \cite{vicinity} presents an efficient randomized algorithm for leader election in large-scale distributed systems. The proposed algorithm is optimal in message complexity ($O(n)$ for a set of $n$ processes), has round complexity logarithmic in the number of processes in the system, and provides high probabilistic guarantees on the election of a unique leader. The algorithm relies on a balls and bins abstraction and works in two phases. The main novelty of the work is in the first phase where the number of contending processes is reduced in a controlled manner. Probabilistic quorums are used to determine a winner in the second phase.
The protocol is completely probabilistic. Do not choose the best represented, but one in a random order.


In \cite{CDC} a peer connectivity-based distributed solution to cluster node is proposed. It assumes each node knowledges only its direct neighbors.
The protocol allows the entire network clustering around a set of starting nodes. The connection structure of a P2P network is represented by a graph where nodes form the vertices and connections between nodes are the branches of the graph.
The algorithm can be extended and used in a weighted graph where the weight associated with a connection between two nodes represents the similarity between the two neighbors. Each node completely ignores the structure of the network. Also consider working on a network of highly dynamic with frequent entry and exit of nodes.
A critical aspect of this solution is that the division of the nodes in clusters depends greatly on the choice of the initial nodes from which the algorithm starts. This may determine that the chosen nodes is significantly different from the ideal one (medoid) to represent the cluster. Also, the number of clusters is fixed, they can evolve only in size (insertion/delete of node in/by the network), new cluster are not created to reflect changing in the structure of the network.
Moreover, the resulting clusters are all at the same level excluding the ability to model sub-categories as described in SONs.

